Hyperbolicity of Alternating Links in Thickened Surfaces with Boundary

Let $F$ be a compact orientable surface with nonempty boundary other than a disk. Let $L$ be a link in $F \times I$ with a connected weakly prime cellular alternating projection to $F$. We provide simple conditions that determine exactly when $(F \times I) \setminus N(L)$ is hyperbolic. We also consider suitable embeddings of $F \times I$ in an ambient manifold $Y$ with boundary and provide conditions on links $L \subset F \times I$ which guarantee tg-hyperbolicity of $Y \setminus N(L)$. These results provide many examples of hyperbolic links in handlebodies and fiber bundles. It also provides many examples of staked links that are hyperbolic.

==> sections/pfpropvol.tex <==
{\color{blue} Do we want to remove this section? With the stronger Theorem 1.8, this seems out of place. But let me know what you think.}As mentioned in the introduction, we can prove a weaker version of Theorem \ref{thm-circle-bundle} using a result of Agol, Storm, and Thurston from \cite{ast}. This result has the advantage of giving a lower bound on volume.

{\color{blue} I don't think the following lemma is necessary. Once you have a tg-hyperbolic manifold, doubling across its boundary must give you a hyperbolic manifold. This is why we can compute volumes, etc. It follows by just extending the metric across the totally geodesic boundary. Lemma comes for free.}

For the proof, we want to show that the manifold $\Tilde{M}$ obtained by ``doubling $M$ across its horizontal boundary" is hyperbolic if $M$ is tg-hyperbolic. More formally: take a copy of $M$ together with a reflected copy $M^R$. The former contains $F \times \{t\}$ for $t \in \{0, 1\}$ and the latter contains reflected versions $F^R \times \{t\}$ for $t \in \{0, 1\}$. Finally glue $F \times \{t\}$ to $F^R \times \{t\}$ for $t \in \{0, 1\}$ via reflection of $F$. Also, let $G$ denote the (disconnected) surface $F \times \{0, 1\} \subset \Tilde{M}$. 

\begin{lemma}
Assume the same hypotheses as Proposition \ref{prop-weak-circle-bundle}. If $M$ is tg-hyperbolic, then $\Tilde{M}$ is hyperbolic and $G$ is totally geodesic in $\Tilde{M}$. 
\end{lemma}

\begin{proof}
By Thurston's Hyperbolization Theorem, it suffices to show there are no essential spheres, tori, disks, or annuli. As usual, we denote such an essential surface by $\Sigma$ and we assume the embedding of $\Sigma$ minimizes $(s, i)$ lexicographically. We consider the subsurfaces of $\Sigma$ resulting from cutting $\Tilde{M}$ along $G$, which recovers $M \sqcup M^R$. \newline 

% not sure if the latex here is okay, or if there's a standard for writing casework like this?
\noindent \textbf{Case 1: $\Sigma$ is a sphere.} Observe that $\Sigma \cap G$ cannot be empty; otherwise, $\Sigma$ is an essential sphere in $M$ or $M^R$. Let $\alpha \subset \Sigma \cap G$ be an intersection curve which is innermost on $\Sigma$: then without loss of generality it bounds a disk in $\Sigma \cap M$. If this disk were $\partial$-parallel, then we can isotope $\Sigma$ to remove $\alpha$ and reduce $i$; hence, $\alpha$ bounds an essential disk in $M$, a contradiction. \newline

\noindent \textbf{Case 2: $\Sigma$ is a disk.} Suppose $\Sigma$ is essential in $\Tilde{M}$ and consider the (nonempty) intersection curves in $\Sigma \cap G$. Let $\alpha \subset \Sigma \cap G$ be a curve which is innermost on $\Sigma$. If $\alpha$ is closed, then $\alpha$ bounds a disk $D \subset G$ by incompressibility and a disk $D' \subset \Sigma$. By irreducibility, $D \cup D'$ is a 2-sphere bounding a 3-ball, and we can isotope $\Sigma$ to remove $\alpha$. Now suppose $\alpha$ is an arc. With an arc $\beta \subset \partial G$, it bounds a disk $D \subset G$ and with an arc $\gamma \subset \partial \Sigma$, it bounds a disk $D' \subset \Sigma$ which, without loss of generality, is properly embedded in $M$. By Lemma \ref{prop-no-essential-disks}, $D'$ must be $\partial$-parallel in $M$; in particular, $\beta \cup \gamma$ bounds a disk $E \subset \partial M$ and $D \cup D' \cup E$ is a 2-sphere bounding a 3-ball. Then we can isotope $\Sigma$ to remove $\alpha$ and assume $\Sigma \cap G$ is empty. Using condition (iii'), we conclude $\Sigma$ must be $\partial$-parallel; hence, $\Tilde{M}$ has no essential disks. \newline 

\noindent \textbf{Case 3: $\Sigma$ is an annulus.} We may assume the intersection curves in $\Sigma \cap G$ are nontrivial on $\Sigma$; otherwise, the innermost trivial curve can be isotoped away as in Case 2. Then the intersection curves are all parallel on $\Sigma$ and cut $\Sigma$ into a collection of either disks or annuli. In the former case, label the disks by $\{D_i\}_{i = 1}^n$ so that $D_i$ and $D_{i + 1}$ intersect in a boundary arc on $F \times \{0\}$ when $i$ is odd and on $F \times \{1\}$ when $i$ is even. Each $D_i$ must be $\partial$-parallel. Then for $i = 1, \dotsc, n$, $\partial D_i$ bounds a disk $E_i$ on $\partial M$, and by irreducibility, $D_i \cup E_i$ bounds a 3-ball $B_i$. Since $F$ is not a disk, the boundary arcs $\partial D_i \cap G$ bound unique disks in $G$, and these disks are the intersection of adjacent $E_i$. Then the $B_i$ glue together along the intersection disks into a solid torus $T$ whose boundary contains $\bigcup_{i = 1}^n D_i = \Sigma$ and $\partial T \setminus \Sigma$ lies in $\partial \Tilde{M}$. Therefore, $\Sigma$ is $\partial$-parallel in $\Tilde{M}$. {\color{purple} maybe will add a figure.....?}

Now suppose $\Sigma \cap G$ cuts $\Sigma$ into a collection of annuli, labelled $\{A_i\}_{i = 1}^n$. By Lemma \ref{prop-no-essential-annuli}, the $A_i$ are either compressible, $\partial$-compressible, and/or $\partial$-parallel in $M$ or $M^R$. Suppose without loss of generality that $A_0$ is $\partial$-parallel in $M$. Then there is an annulus $A$ in $M$ with one boundary component on $A_0$ isotopic to a core curve of $A_0$ and another boundary component on $\partial F \times I$ also isotopic to a core curve. Perform an \textit{annular compression} on $\Sigma$ along $A$, yielding two essential annuli in $\Tilde{M}$. After performing finitely many of these annular compressions, we may take $\Sigma$ to be one of the resulting annuli and henceforth assume that none of the $A_i$ are $\partial$-parallel in $M$ (or $M^R$). Also, if any of the $A_i$ are compressible, then $\Sigma$ is compressible. Hence, all of the $A_i$ must be $\partial$-compressible in $M$ (or $M^R$). 

We claim that $\Sigma$ must be $\partial$-compressible in $\Tilde{M}$. For $i = 1, \dotsc, n$, let $\gamma_i$ be an arc properly embedded in $A_i$ and let $\beta_i$ be an arc properly embedded in $\partial M$ (or $\partial(M^R)$) so that $\beta_i \cup \gamma_i$ bounds a $\partial$-compression disk $D_i$ in $M$ (or in $M^R$). We may isotope the $D_i$ in $M$ and $M^R$ so that each pair of adjacent arcs $\gamma_i$ and $\gamma_{i + 1}$ share an endpoint and the corresponding disks $D_i$ and $D_{i + 1}$ share boundary in $G$. Then when reconstructing $\Sigma = \bigcup_{i = 1}^n A_i$, the $\gamma_i$ and $D_i$ glue together to result in a $\partial$-compression disk $D = \bigcup_{i = 1}^n D_i$ for $\Sigma$ with arc $\Sigma \cap D = \bigcup_{i = 1}^n \gamma_i$. Hence, $\Tilde{M}$ has no essential annuli. \newline 

\noindent \textbf{Case 4: $\Sigma$ is a torus.} If $\Sigma \cap G$ is empty, then after cutting along $G$, without loss of generality $\Sigma$ is a torus in $M$ which is incompressible and, using condition (iii'), not $\partial$-parallel. Hence, we may assume $\Sigma \cap G$ is not empty. Again, we may assume the intersection curves in $\Sigma \cap G$ are nontrivial on $\Sigma$; otherwise, we may isotope them away using incompressibility of $G$. Hence, the intersection curves are parallel $(p, q)$-curves on $\Sigma$, and  they slice $\Sigma$ into a collection $\{A_i\}_{i = 1}^n$ of annuli lying in $M$ and $M^R$. 

By Lemma \ref{prop-no-essential-annuli}, the $A_i$ are either compressible, $\partial$-compressible, and/or $\partial$-parallel in $M$ or $M^R$. We may assume the $A_i$ are all incompressible in $M$ (or $M^R$): otherwise, we can find a compressing disk for $\Sigma$. If, without loss of generality, $A_0$ is $\partial$-parallel in $M$, then we may perform an annular compression on $\Sigma$ which yields an essential annulus $\Sigma'$ in $\Tilde{M}$, contradicting Case 3. Hence, the $A_i$ are all $\partial$-compressible, with $\partial$-compression disks $D_i$ bounded by arcs $\gamma_i \subset A_i$. The $D_i$ glue together into an annulus $A = \bigcup_{i = 1}^n D_i$ with one boundary component on $\partial \Tilde{M}$ and one boundary component on $\Sigma$ running transverse to the curves in $\Sigma \cap G$. Perform an annular compression on $\Sigma$ along $A$, resulting in an essential annulus. This contradicts Case 3. \newline 

Now the lemma follows from Thurston's Hyperbolization Theorem. Also, $G$ is totally geodesic since it is the fixed point set of the reflection map exchanging $M$ and $M^R$. 
\end{proof}

\begin{proof} [Proof of Proposition \ref{prop-weak-circle-bundle}]
By Theorem \ref{thm-thickened} and condition (iii'), we know that $M = (F \times I) \setminus N(L)$ must be tg-hyperbolic. Suppose that in the construction of $M'$ the ambient manifold $F \Tilde{\times} S^1$ was formed by identifying $F \times \{0\}$ and $F \times \{1\}$ via the orientation-preserving self-homeomorphism $\varphi: F \to F$. Then let $\Tilde{M'}$ denote the covering space of $M'$ obtained in the following way. Take two copies of $M$ denoted $M_1$ and $M_2$. Each contains a copy of $F \times \{t\}$, for every $t \in \{0, 1\}$, and we denote these by $F_i \times \{t\}$ for $i = 1, 2$. We glue $F_1 \times \{1\}$ to $F_2 \times \{0\}$ according to $\varphi$ and glue $F_2 \times \{1\}$ to $F_1 \times \{0\}$ also according to $\varphi$. We call the resulting manifold $\Tilde{M'}$, and it is a 2-sheeted covering space for $M'$. In particular, it is hyperbolic if and only if $M'$ is hyperbolic. 

By the previous lemma, the manifold $\Tilde{M}$ is hyperbolic and contains a totally geodesic surface $G$. By Theorem 7.2 of \cite{ast} and its extension Theorem 5.5 of \cite{cfw}, any manifold obtained from $\Tilde{M}$ by cutting along $G$ and regluing along some self-homeomorphism of $G$ yields a manifold which is also hyperbolic and whose volume is greater than or equal to the volume of the original manifold. In our situation, we cut along $G$ yields four copies of $F$, namely, $F \times \{t\}$ and $F^R \times \{t\}$ for $t = \{0, 1\}$. Then we glue $F \times \{0\}$ to $F^R \times \{1\}$ via $\phi$ precomposed with reflection and similarly glue $F \times \{1\}$ to $F^R \times \{0\}$. See Figure \ref{fig-gluing-ast}. 

\begin{figure} [htbp]
    \centering
    \includegraphics[scale=.5]{figures/volumegreater.pdf}
    \caption{We cut and reglue along $G$ to obtain $\Tilde{M}'$ from $\Tilde{M}$.}
    \label{fig-gluing-ast}
\end{figure}

This recovers $\Tilde{M}'$; hence, if $M$ is tg-hyperbolic, $\Tilde{M}'$ is hyperbolic and so is $M'$. Moreover, by \cite{ast} and \cite{cfw} we know that
\begin{align*}
    \vol(M') = \frac{1}{2} \vol(\Tilde{M}') \geq \frac{1}{2} \vol(\Tilde{M}) = \vol(M)
\end{align*}
with equality if and only if $G$ is also tg-hyperbolic in $\Tilde{M}'$. 
\end{proof}



